On Plans With Loops and Noise

In an influential paper, Levesque proposed a formal specification for analysing the correctness of program-like plans, such as conditional plans, iterative plans, and knowledge-based plans. He motivated a logical characterisation within the situation calculus that included binary sensing actions. While the characterisation does not immediately yield a practical algorithm, the specification serves as a general skeleton to explore the synthesis of program-like plans for reasonable, tractable fragments. Increasingly, classical plan structures are being applied to stochastic environments such as robotics applications. This raises the question as to what the specification for correctness should look like, since Levesque's account makes the assumption that sensing is exact and actions are deterministic. Building on a situation calculus theory for reasoning about degrees of belief and noise, we revisit the execution semantics of generalised plans. The specification is then used to analyse the correctness of example plans.

==> On Plans With Loops and Noise/defn.tex <==


                                                        
                                                        


%theorem

%black box
\newcommand{\bbox}{\vrule height7pt width4pt depth1pt}
%\newcommand{\eprf}{\bbox\vspace{0.1in}}
%\newcommand{\qed}{\eprf}
% (not)member of
\let\member=\in
\let\notmember=\notin
% \sub will be used for subscript.
\newcommand{\sub}{_}
% \su will be used for superscript.
\def\su{^}
%right arrow
\newcommand{\rarrow}{\rightarrow}
\newcommand{\raw}{\rarrow}
\newcommand{\goto}{\raw}
%\newcommand{\goto}{\rarrow}
%left arrow
\newcommand{\larrow}{\leftarrow}

\newcommand{\real}{{\mathbb{R}}}
\newcommand{\nat}{{\mathbb{N}}}
%double turnstile
%\newcommand{\sat}{\models}
\newcommand{\dtur}{\models}
%single turnstile
\newcommand{\infers}{\vdash}
\newcommand{\stur}{\vdash}
\newcommand{\done}{{\it stop}}
%fat right arrow
\newcommand{\rimp}{\Rightarrow}
%fat left arrow
\newcommand{\limp}{\Leftarrow}
%fat double arrow
\newcommand{\dimp}{\Leftrightarrow}
%big or
\newcommand{\bor}{\bigvee}
\newcommand{\know}{{\it Know}}
\newcommand{\bel}{{\it Bel}}
%big and
\newcommand{\band}{\bigwedge}
%union
\newcommand{\union}{\cup}
%intersection
\newcommand{\inter}{\cap}
%bold letters
\newcommand{\xx}{{\bf x}}
\newcommand{\yy}{{\bf y}}
\newcommand{\uu}{{\bf u}}
\newcommand{\vv}{{\bf v}}
\newcommand{\FF}{{\bf F}}
\newcommand{\natnum}{{\sl N}}
%\newfont{\sqi}{cmssqi8}

\newcommand{\lt}{<}
\newcommand{\gt}{>}
\newcommand{\all}{\forall}
\newcommand{\infinity}{\infty}
%binomial coefficient:

\newcommand{\bigfootnote}[1]{{\footnote{\normalsize #1}}}
\newcommand{\medfootnote}[1]{{\footnote{\small #1}}}
\newcommand{\bd}{\bf}

% Joe's Section

\newcommand{\imp}{\Rightarrow}

%\H, \L, \O, \P and \S already taken; but we're redefining \P anyway
\newcommand{\A}{{\cal A}}
\newcommand{\B}{{\cal B}}
%\newcommand{\C}{{\cal C}}
\newcommand{\D}{{\cal D}}
\newcommand{\E}{{\cal E}}
\newcommand{\F}{{\cal F}}
%\newcommand{\G}{{\cal G}}
%\newcommand{\H}{{\cal H}}
\newcommand{\cal}{\mathcal}
\newcommand{\init}{{\it Init}}
\newcommand{\ivar}{{\iota}}
\newcommand{\I}{{\cal I}}
\newcommand{\J}{{\cal J}}
\newcommand{\K}{{\cal K}}
\renewcommand{\L}{{\cal L}}
\newcommand{\M}{{\cal M}}
\newcommand{\N}{{\cal N}}
\renewcommand{\O}{{\cal O}}
\newcommand{\Ocal}{{\cal O}}
\newcommand{\Hcal}{{\cal H}}
\renewcommand{\P}{{\cal P}}
\newcommand{\Q}{{\cal Q}}
\newcommand{\obs}{{\it SF}}
\newcommand{\R}{{\cal R}}
\renewcommand{\S}{{\cal S}}
\newcommand{\fsa}{\mathit{\Sigma}}
\newcommand{\T}{{\cal T}}
%\newcommand{\U}{{\cal U}}
\newcommand{\V}{{\cal V}}
\newcommand{\W}{{\cal W}}
\newcommand{\X}{{\cal X}}
\newcommand{\Y}{{\cal Y}}
\newcommand{\Z}{{\cal Z}}
\newcommand{\ti}{\textit}
\newcommand{\Kone}{{\cal K}_1}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\Ki}{{\cal K}_i}
\newcommand{\Kn}{{\cal K}_n}
\newcommand{\st}{\, \vert \,} %vertical bar with space around it
\newcommand{\stc}{\, : \,} %colon with space around it
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newtheorem{nlem}{Lemma}
\newtheorem{Ob}{Observation}
\newtheorem{pps}{Proposition}
\newtheorem{defn}{Definition}
\newtheorem{crl}{Corollary}
\newtheorem{cl}{Claim}
\newcommand{\pf}{\par\noindent{\bf Proof}~~}
\newcommand{\eg}{\emph{e.g.}~}
\newcommand{\ie}{\emph{i.e.}~}
\newcommand{\vs}{vs.~}
\newcommand{\cf}{cf.~}
\newcommand{\etal}{et al.\ }
\newcommand{\resp}{resp.\ }
\newcommand{\respc}{resp.,\ }
%\newcommand{\comment}[1]{\marginpar{\scriptsize\raggedright #1}}
\newcommand{\wrt}{with respect to~}
\newcommand{\re}{r.e.}
\newcommand{\If}{{\bf if}}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\qinit}{{Q_0}}
\newcommand{\qi}{{Q\sub 0}}
\newcommand{\qf}{{Q\sub F}}
\newcommand{\wi}{{w\sub 0 }}
%\newcommand{\next}[1]{\xrightarrow{ #1}}
\newcommand{\poss}{\ti{Poss}}
\newcommand{\sr}{\ti{SR}}
\newcommand{\qfinal}{{Q_F}}
\newcommand{\qmin}{\Q^-}
\newcommand{\ins}{{S_{0}}}
\renewcommand{\ss}{{s^*}}
\newcommand{\thereis}{\exists}
\newcommand{\is}{\thereis}
\newcommand{\chop}{\emph{chop}}
\newcommand{\move}{\emph{move}}
\newcommand{\fwd}{\emph{fwd}}
\newcommand{\xpos}{\emph{h}}
%\newcommand{\tr}{\textit{T}}
\newcommand{\ts}{{T^*}}%{{\tr^*}}
\newcommand{\alt}{\textit{alt}}
\newcommand{\Then}{{\bf then}}
\newcommand{\Until}{{\bf until}}
\newcommand{\Else}{{\bf else}}
\newcommand{\Repeat}{{\bf repeat}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cI}{{\cal I}}
%\newcommand{\IcR}{{\cal I}_{\cal R}}
%\newcommand{\IRca}{{\cal I}_\Rca}
%\newcommand{\Rca}{{\cR_{ca}}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}

\newcommand{\true}{\mbox{{\it true}}}
\newcommand{\false}{\mbox{{\it false}}}


